Sketch2Stress: Sketching with Structural Stress Awareness

In the process of product design and digital fabrication, the structural analysis of a designed prototype is a fundamental and essential step. However, such a step is usually invisible or inaccessible to designers at the early sketching phase. This limits the user's ability to consider a shape's physical properties and structural soundness. To bridge this gap, we introduce a novel approach Sketch2Stress that allows users to perform structural analysis of desired objects at the sketching stage. This method takes as input a 2D freehand sketch and one or multiple locations of user-assigned external forces. With the specially-designed two-branch generative-adversarial framework, it automatically predicts a normal map and a corresponding structural stress map distributed over the user-sketched underlying object. In this way, our method empowers designers to easily examine the stress sustained everywhere and identify potential problematic regions of their sketched object. Furthermore, combined with the predicted normal map, users are able to conduct a region-wise structural analysis efficiently by aggregating the stress effects of multiple forces in the same direction. Finally, we demonstrate the effectiveness and practicality of our system with extensive experiments and user studies.

==> figures/fig_network_details_supple.tex <==
\begin{figure}[htbp]{
    \centering
    \includegraphics[width=.98\linewidth]{figures/network_details.pdf}
    \caption{The details of our two-branch Sketch2Stress network. The block of \textit{Conv}/\textit{Upconv}/\textit{Deconv} \textit{(input\_channel\_number, output\_channel\_number, kernel\_size, stride, padding\_width)} respectively represents Convolution, Upsampling $+$ Convolution, and Deconvolution layer. 
    Note that each Conv/Upconv/Deconv layer is followed by leaky ReLU and batch normalization, which are omitted in the figure for simplicity.
    }
    \label{fig:network_details_supple}
    }
\end{figure}

==> figures/fig_supplemental_qualititive.tex <==
\begin{figure*}[t]{
    \centering
    % \vspace{-5mm}
    \includegraphics[width=\linewidth]{figures/qualitative_supple_A.pdf}
    \caption{Qualitative comparison of {results generated by} %generation results of 
    different methods of pix2pix, pix2pixHD, our method, and ground truth.
    The leftmost column {shows} %s are 
    the input sketches and the external forces (plotted as red dots on sketches). 
    }
   
    \label{fig:qualtative_supple_A}
    }
\end{figure*}


\begin{figure*}[t]{
    \centering
    % \vspace{-5mm}
    \includegraphics[width=\linewidth]{figures/qualitative_supple_B.pdf}
    \caption{Qualitative comparison of {results generated by} %generation results of 
    different methods of pix2pix, pix2pixHD, our method, and ground truth.
    The leftmost column {shows} %s are 
    the input sketches and the external forces (plotted as red dots on sketches).  
    }
   
    \label{fig:qualtative_supple_B}
    }
\end{figure*}

\begin{figure*}[t]{
    \centering
    % \vspace{-5mm}
    \includegraphics[width=\linewidth]{figures/qualitative_supple_C.pdf}
    \caption{Qualitative comparison of {results generated by} 
    different methods of pix2pix, pix2pixHD, our method, and ground truth.
    The leftmost column {shows} %s are 
    the input sketches and the external forces (plotted as red dots on sketches).  
    }
   
    \label{fig:qualtative_supple_C}
    }
\end{figure*}

==> figures/fig_supplemetal_comparison.tex <==
\begin{figure}[t]{
    \centering
    % \vspace{-5mm}
    \includegraphics[width=\linewidth]{figures/supplemental_comparison_qualitative.pdf}
    \caption{{Compared with some variants of our proposed method. {Please see the sketch and specified force point in Figure 11 of the main paper.} 
    }}
\label{fig:supplemental_qualtative_comaparison}
    }
\end{figure}






==> sections/supplemental_abstract.tex <==
\begin{abstract}


\end{abstract}  

==> sections/supplemental_content.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=1\linewidth]{figs/supplemental_network_im.pdf}
    \caption{\label{fig:fig_supple_sketch_im_network}
            Network structure of the sketch implicit model.}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=1\linewidth]{figs/supplemental_network_assembly.pdf}
    \caption{\label{fig:fig_supple_sketch_assembly_network}
            Spatial transformation network (STN) for sketch assembly.}
\end{figure}



\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/fig_supplemental_fig1_v2.pdf}
    \caption{\label{fig:fig_supple_more_results1}
           Visual results of our method. Each triplet contains an input sketch (Left), the sketch after part beautification (Middle), and the final result after structure beautification (Right). Please zoom in for better visualization.}
\end{figure*}

\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/fig_supplemental_fig2_v2.pdf}
    \caption{\label{fig:fig_supple_more_results1}
        Visual results of our method. Each triplet contains an input sketch (Left), the sketch after part beautification (Middle), and the final result after structure beautification (Right). Please zoom in for better visualization. }
\end{figure*}


\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/fig_supplemental_fig3_v3.pdf}
    \caption{\label{fig:fig_supple_more_results1}
        Visual results of our method. Each triplet contains an input sketch (Left), the sketch after part beautification (Middle), and the final result after structure beautification (Right). Please zoom in for better visualization.}
\end{figure*}
